Using Anomaly Feature Vectors for Detecting, Classifying and Warning of Outlier Adversarial Examples

We present DeClaW, a system for detecting, classifying, and warning of adversarial inputs presented to a classification neural network. In contrast to current state-of-the-art methods that, given an input, detect whether an input is clean or adversarial, we aim to also identify the types of adversarial attack (e.g., PGD, Carlini-Wagner or clean). To achieve this, we extract statistical profiles, which we term as anomaly feature vectors, from a set of latent features. Preliminary findings suggest that AFVs can help distinguish among several types of adversarial attacks (e.g., PGD versus Carlini-Wagner) with close to 93% accuracy on the CIFAR-10 dataset. The results open the door to using AFV-based methods for exploring not only adversarial attack detection but also classification of the attack type and then design of attack-specific mitigation strategies.

==> 012_related.tex <==
\section{Related Work}
\label{Section:RelatedWork}

Existing detection techniques span a wide variety of approaches. One approach converts last couple layers of a neural network into Bayesian layers~\cite{deng2021libre} while another does neural fingerprinting~\cite{dathathri2018detecting}. More common techniques include training a second-stage classifier~\cite{grosse2017statistical,gong2017adversarial,metzen2017detecting,aigrain2019detecting}, detecting statistical properties~\cite{bhagoji2017dimensionality,hendrycks2016early,li2017adversarial,crecchi2019detecting, pang2017towards}, and running statistical tests~\cite{grosse2017statistical,feinman2017detecting,roth2019odds}. We aim to build statistical AFVs and run both detection of attacks and classification of the type of attack.




To simplify the detection decision, detectors rely on generating an alternative 
(often high dimensional) embedding space over which to project natural and adversarial examples
into manifolds where to then discern boundaries or nearest neighbors. 
By comparing histograms from adversarial examples against that of natural examples, we compose
anomaly detection features to span such manifolds based on magnified discrepancies between those histograms.  Using an anomaly-oriented statistical profile to produce an embedded space, 
we also leverage KNN distances~\cite{cohen2020detecting, papernot2018deep} to both neighboring natural and adversarial examples to train the detector neural network. 
However, although these approaches claim high accuracy for several attack methods, 
they require an iterative DkNN training phase which is computational expensive. Similarly, unlike the kernel density estimation in ~\cite{pang2018robust}, our approach approximates KDE features using inexpensive histogram comparison analysis while again requires no training on the pretrained model being defended -- only evaluation mode access.



% \subsection{Distributional Defenses}
%Attack detectors represent a form of distribution-based defenses where features from input samples are compared to corresponding features from natural inputs assumed to be perturbation-free or clean. Nevertheless, poisoning attacks are possible, so a defense that can also detect not only attacks but also out of distribution samples to purify the training dataset. 



%\rf{Which paper is this referring to?} Previous work construct statistical test point-estimates for differentiating between two distributions. We use an anomaly detection approach. Classical Gaussian anomaly detection relies on plus/minus $3\sigma$ for constructing anomaly upper and lower ($LCL, UCL$) decision boundaries. Well-known tests are used to test for difference in various statistical moments and point estimates between the two sampled populations.
%Even though we sample the inputs to a hidden layer, we differ on these in terms of the granularity of the sampled populations we consider for many multiple comparison-based features, the types of tests we apply (e.g., histogram comparison, area ratios, and what inputs we consider as our foundational sampling population. %Whereas previous work on detectors have been reported to achieve accuracy of X\%, using these enhancements, we have achieved accuracy of Y\%.



 In ~\cite{metzen2017detecting}, 
 %a GAN is used to generate a generative distributional profile of the natural samples. 
 %IMPORTANT THIS IS QUOTED TEXT TAKEN STRAIGHT FROM THE ADVERSARIAL PERTURBATIONS PAPER.
 %\rf{rewrite to provide 2-5 sentence summary of what these papers did, followed by a 2-3 sentence summary that explains how we are different from them}
 %\begin{quote}
 the authors also train a binary detector.  The detector is fed inputs from intermediate feature representations of a classifier, to discriminate between samples from the original data set and adversarial examples. 
 %Being able to detect adversarial perturbations might help in safety- and security-critical semi-autonomous systems as it would allow disabling autonomous operation and requesting human intervention (along with a warning that someone might be manipulating the system).
 %However, it might intuitively seem very difficult to train such a detector since adversarial inputs are generated by tiny, sometimes visually imperceptible, perturbations of genuine examples. 
Their results on CIFAR10 assert that their detector achieves $91.3\%$ accuracy in detection of adversarial inputs. 
Moreover, while the authors train the detector to detect perturbations of a specific adversary, the authors assert that the detector generalizes to similar and weaker adversaries. 
%\end{quote}



% "In this section, we give a brief introduction to the key components of model attacks and defenses. We hope that our explanations can help our audience to understand the main components of the related works on adversarial attacks and their countermeasures."


% IMPORTANT THIS IS QUOTED TEXT TAKEN STRAIGHT FROM THE ADVERSARIAL PERTURBATIONS PAPER.

%"As Szegedy et al. (2014) have shown, small but carefully directed perturbations of images can lead to incorrect classification with high confidence on artificial systems. Yet, for humans these perturbations are often visually imperceptible and do not stir any doubt about the correct classification. In fact, so called adversarial examples are crucially characterized by requiring minimal perturbations that are quasi-imperceptible to a human observer.

% Several approaches exist to increase a model’s robustness against adversarial attacks. Goodfellow et al. (2015) propose to augment the training set with adversarial examples. At training time, they  minimize the loss for real and adversarial examples, while adversarial examples are chosen to fool the current version of the model. In contrast, Zheng et al. (2016) propose to append a stability term to the objective function, which forces the model to have similar outputs for samples of the training set and their perturbed versions. This differs from data augmentation since it encourages smoothness of the model output between original and distorted samples instead of minimizing the original objective on the adversarial examples directly. Another defense-measure against certain adversarial attack methods is defensive distillation (Papernot et al., 2016b), a special form of network distillation, to train a network that becomes almost completely resistant against attacks such as the L-BFGS attack (Szegedy et al., 2014) and the fast gradient sign attack (Goodfellow et al., 2015). However, Carlini \& Wagner (2016) recently introduced a novel method for constructing adversarial examples that manages to (very successfully) break many defense methods, including defensive distillation. In fact, the authors find that previous attacks were very fragile and could easily fail to find adversarial examples even when they existed. An experiment on the cross-model adversarial portability (Rozsa et al., 2016) has shown that models with higher accuracies tend to be more robust against adversarial examples, while examples that fool them are more portable to less accurate models






Existing detection techniques span a wide variety of approaches. One approach converts last couple layers of a neural network into Bayesian layers~\cite{deng2021libre} while another does neural fingerprinting~\cite{dathathri2018detecting}. More common techniques include training a second-stage classifier~\cite{grosse2017statistical,gong2017adversarial,metzen2017detecting,aigrain2019detecting}, detecting statistical properties~\cite{bhagoji2017dimensionality,hendrycks2016early,li2017adversarial,crecchi2019detecting}, and running statistical tests~\cite{grosse2017statistical,feinman2017detecting,roth2019odds}. We aim to build statistical AFVs and run both detection of attacks and classification of the type of attack.



\js{
The authors in ~\cite{bhagoji2017dimensionality} improve the robustness of ML classification and training phases against evasion attacks by reducing data dimensionality. Although a few different distinct types of attacks have been selected from the literature in their threat model, the paper only focuses on the defense against attacks across multiple ML classifier, whereas DeClaw focuses on how to differentiate and detect different groups of attacks. 

~\cite{dathathri2018detecting} encodes fingerprint patterns into the response of a DNN around real data, which characterize the DNN’s expected behavior around real data and can later be used to detect adversarial examples (similar to the idea of Dynamic Watermarking). However, fingerprint-based approach does require encoding certain features into the data distribution in a proactive way, and it does not differentiate different class of attacks like DeClaw. 

~\cite{gong2017adversarial} also looks into disparity among adversarial samples. However, this work only studies 3 attacks (FGSM, TGSM and JSMA) and authors also admitted that "FGSM and JSMA generate adversarial datasets that are far away from each other. But it is too vague without defining precisely what is being far away". In contrast, DeClaw studies 11 different types of attacks. DeClaw also compares and differentiates them using a more quantitative distribution approach, which potentially leads to a more accurate and effective way for anomaly detection. One detection method proposed in 

~\cite{li2017adversarial} is based the observation that correctly classified and many out-of-distribution examples tend to have different softmax distributions. However, this paper did not focus on the attack classification, nor study how exactly the distribution are different caused by different type of adversarial attacks. 

In~\cite{aigrain2019detecting}, the authors augmented classification by branching off the main network at certain layer, and then this subnetwork detector is trained on the adversarial input and produce an output which is interpreted as the probability of the input being adversarial. However, the paper only compares the accuracy of the detector against 4 different adversaries with the focus more on their detector, rather than categorizing different type of attacks based on their distributional characterization. 

The authors in~\cite{cohen2020detecting} distinguishes adversarial examples on six attack methods (FGSM, JSMA, Deepfool, CW, PGD,and EAD) based on the observation that the impact of training samples on the validation set data are different. By fitting a k-NN model on the DNN's activation layers, the
authors shows that the samples are highly correlated with the nearest neighbors of the normal inputs, while this correlation is much weaker for adversarial inputs. However, the work does not address how to identify different types of adversarial attacks based on these k-NN features.

The proposed method in~\cite{yang2019mlloo} is based on the observation that the feature attribution map of an adversarial example near the boundary always differs from that of the corresponding clean example. The authors also use statistical dispersion in feature attribution to detect 6 different adversarial examples. However, compared to DeClaw, this approach is focused on the confidence level rather than distributional characterization of different attacks. Therefore, it does not help classify and differentiate different attacks.
}







==> 03_goals.tex <==
\section{Motivating Goals}
\label{Section:MotivatingGoals}


Within the domain of image classification, adversarial examples are generally modeled as noise perturbations over natural examples (e.g., seemingly apparent random noise over an image) that force a classification error. This is referred to as an evasion attack. Another more subtle form of an adversarial example is a poisoning attack, where the attacker is able to poison the natural training samples with examples to distort the decision boundaries of the resulting model. %\rf{other detection papers make the case that making models that can correctly handle adversarial examples is difficult and thus detection becomes a useful alternative. A similar argument here may be helpful}.  
While developing robust models to handle adversarial inputs is difficult, new attack methods keep emerging. Therefore, a detection technique becomes a useful defense option. In particular, it would be desirable to obtain a defense that could identify:
\begin{itemize}
\item adversarial examples during classification (e.g., evasion)
\item adversarial examples during training (e.g., poisoning)
\item out of distribution, low confidence examples during classification (e.g., samples with very low or null trained classification support)
\item out of distribution, high distortion examples during training (e.g., samples with very high anomaly scores).
\end{itemize}


%Moreover, it would be desirable if training a defense would not require very large data sets but perhaps a normative slice of the data.
%\js{Really interesting categorization. This also makes me think whether the size of data set will have any impact to DeClaw's accuracy. For example, I saw some papers in the past about how to achieve accurate classification with very small data set. Will FPR be related to the size of dataset? This could be very useful to AV since it is currently still impractical to collect all possible data.}









==> 04_vision.tex <==
\begin{figure}
\centerline{
\includegraphics[width=0.3\textwidth]{FIGURES/augmented_model.png}}
\caption{%PLACEHOLDER: Just in case Prof. Prakash wants a vision statement here aligned to his integrative positioning of robust ML. "
Our grand vision is towards the augmentation of online classification models from a logit/probability output into robust machine learning ensembles with advisory signals 
% (and reactive logic (no shown)) 
that through introspection over learned concepts and observed input distributions enforces process control of the online classification pipeline, for example,
(1) raises an alarm for human operator intervention if needed, 
(2) reliably detects and identifies anomalous inputs as well as adversarial inputs
(3) quantifies the classification support of generated predictions and 
(4) otherwise, autonomously processes confident classifications.}
\label{vision_augmented_models}
\end{figure}





\subsection{Grand Vision}
\label{Section:GrandVision}


Fig.~\ref{vision_augmented_models} depicts our vision for augmenting classifier models with robust introspection features. In particular, these intelligent classifier qualification (shadow/second-stage) pipelines are foreseeable to be dominant in the automotive domain. Early detection and classification of adversarial inputs during early stages in a pipeline would allow the machine learning to reflect on the sample and speculate:
\begin{itemize}
    \item is the sample out-of-distribution? e.g., a sample may represent a statistical outlier with respect to a normative set of natural samples.
    \item is the sample anomalous? e.g., a sample could exhibit patterns of statistical departures from normative natural samples --- yet without being a statistical outlier.
    \item is the sample adversarial? e.g., a sample may align to existing statistical profiles, clusters, etc for known (or representative) attack samples.
    \item is there confidence that the sample aligns to concepts previously assimilated? e.g., a sample may align to an existing concept from the training data for which a number of similar samples reassert a support for the classification decision.
    \item is the collection of samples indicative of a process shift from the concepts previously assimilated? e.g., a stream of samples that drift away from concepts learned from the training data into a different concept may now raise a warning signal.% daytime vs nighttime concept shift as well as drift. highway vs city driving. 
\end{itemize}

A system (e.g., Declaw) providing answers to these questions would allow the defended machine learning intelligence, to adapt, retrain, warn and/or redirect samples to appropriate remedial measures such as human intervention, alternative models/weights, leverage of ensembles, etc.





% \subsection{Declaw: Detector and Classifier}\label{DETE}






==> 08_profile.tex <==
\subsubsection{Distributional Characterization}\label{CHAR}
In~\cite{metzen2017detecting}, a binary classifier for detection attacks was built by feeding the latent variables at selected intermediate stage, to a separate CNN.
This approach was able to detect with $91\%$ accuracy, the presence of attacks on three attack classes:
PGD, BIM, DeepFool.  
Rather than feeding the latent variables to the secondary neural net, we propose feeding a more compact intermediary representation centered around anomaly detection. The specific features of this intermediary representation are discussed next. Our approach achieves a detection rate of $95.3\%$ and a classification rate of $93\%$ with FPR and FNR rates below $5\%$ --- while classifying not three but rather eleven different attacks (three PGD variants, FGM, BIM. CWL2, DeepFool, Spatial Transform, Square Attack, Wasserstein, and Newtonfool).



Distributional A/B tests (e.g., difference in means, heterogeneity of variances, normality of distributions, etc) are typically weakened by virtue of relatively minute perturbations induced by modern attacks. Naive application of these techniques is usually ineffective. We augment the above with a number of fine-grained anomaly-oriented features that seek to magnify various types of observed discrepancies between the distribution layer values associated with natural samples and the distribution of layer values associated with attacked samples. These techniques are summarized in the subsections below.












\subsubsection{Region-based Aggregated Anomaly Counting Features}
Anomaly counting features divide the observed histogram (i.e., estimated probability density function) of the selected layer inputs into three regions: 
\begin{itemize}
    \item (L, anomaly detection left tail): $\mu - k\sigma$, 
    \item (R, anomaly detection right tail): $\mu + k\sigma$, and 
    \item (C, non-anomalous center): $mu - \sigma \le x_i  \le \mu + k\sigma$.
\end{itemize}
% Fig.~\ref{} illustrates that these tests try to identify anomalies on deviation of the expected traits of the normal distribution for layer inputs for natural samples ($~N(0,1)$).





Traditionally anomaly detection relies on $k=3$ for identifying single statistically significant outliers in a signal. However, our goal here is to determine whether the population of observed layer values as a whole is anomalous with regards to the expected population of values averaged across $10K$ natural samples. For this reason, our goal is to aggregate indicators across each of these (L, C, R) regions. Moreover, we use a value $k=1$ to magnify small anomalies -- statistically, we expect $65\%$ of all values to fall into C whereas approximately $17\%$ each will fall into regions L and R. For each region. we count the total number of values in the region, the average zscore for these values, the total sum of zscores, and various ratio between regions. 
Fig.~\ref{}\rf{what is this supposed to point to?} illustrates that basic idea. Layer inputs are z-scored and considered as a single population. with a histogram built for the zscore values.







\subsubsection{Extreme Value Features}
In addition of these features, given the current layer values, we perform anomaly detection tests that compare these anomaly-detection signal values against for $10$ percentile and $90$ percentile extracted from the population of such signal values across all $10K$ natural samples. These per-region anomaly counting tests examine whether the current layer inputs when considered as a population exhibits extreme values.

%\input{TABLES/table_profile_natural}





\subsubsection{Histogram Bin Count Features}
Histogram binning features represent raw histogram binning counts that estimate the probability density function of the layer inputs $x_i$ across all channels.






\subsubsection{Histogram Tail Symmetry Features}
Symmetry features are used to quantify the symmetry between tail bins. Whereas the probability density function for natural samples is normally distributed, some attack notoriously generate layer inputs for which its probability density function although resembles the expected bell curve exhibits tail symmetry anomalies. These features quantifies differences on bin counts at corresponding positions on both tails of the sampled histogram for the layer inputs $x_i$.




\subsubsection{Statistical Test Features}
Statistical tests are used to generate p-values from the resulting tests (e.g., comparison of means, normality, same distribution, ratio of variances) between (A) a subsample from the population of layer inputs $x_i$ for the underlying image and (B) a subsample from the population of average valuesfor the same layer ---but averaged across the collection of $10K$ natural inputs. These tests examine whether statistical point estimators for the current layer inputs (when considered as a population) are statistically different from the observed estimators computed across the population of $10K$ natural samples.  In general, as the size of subsample being tested grows larger, these tests lose significance. For this reason, tests are conducted using a small size subsample from both populations being tested.





\subsubsection{Similar Shape Probability Distribution Features}
The Wasserstein distance is used to quantify how symmetric are similar are (regions of) binned distributions. In a nutshell, given two k-binned histograms, the Wasserstein distance estimates the work cost of making the skyline on one histogram resemble the other skyline by optimally removing/adding/moving from a mismatching bin into other adjacent bin(s). The larger the metric the larger the "work" (i.e., material over distance) needed to make the distributions look alike. Similar distributions have low distances. Moreover, the distance can be use to analyze symmetry in the tail regions of our distributions.
%\rf{Note: PCA/LDA features do not have their own dedicated section. This breaks parallelism / consistent format}


\subsubsection{Dimensionality Reduction Features}
We also leverage PCA and LDA dimensionality reduction components as features to test whether explicit the induced separability by these projections improve classification accuracy. Fig.~\ref{lda} shows a plot showing the manifold manifested by the first two LDA components for the space spanned by AFVs.



\subsubsection{Nearest Neighbor: Proximity to Known Example Features}
A Radius Nearest Neighbor classifier is used to generate radius neighbor probabilities as features. Let $f_{i}$ be the $i^{th}$ anomaly feature vector with corresponding label $y_i$. Then Radius Nearest Neighbor produces
   $f_i[k]= \sum_{k \in Q}{distance(f_i, f_j) \le r}$.
   
These features represent the ratio ($\frac{A}{B}$) of (A) nearby class members of some class $k$ over (B) the total of neighboring points with a given radius across all classes in $Q$. Notably, the classification is done using standard scaler inputs to preserve outlier anomalies. Using a grid search, a radius of $r=0.7$ (i.e., standard deviations) was found to deliver the best accuracy. Outliers having no neighbors are defaulted to the most frequent class.

As these features examine the peering radius neighborhood of every sample, they help our classifier identify out-of-distribution examples.  Given $Q+1$ classes in our attack classification problem, a Nearest Neighbor is trained with a subsample of the training set and predictions are computed for the entire training set. Given a large enough subsample, $Q+1$ class probabilities will be generated. These probabilities represent the nearest neighbor votes for a radius $r$ from the given sample. These help the classification support for in-distribution samples as well as help identify out-of-distribution outliers (i.e., those feature vectors having no neighbor counts).










==> 10_ablation.tex <==
\section{Ablation Studies}
\label{Section:AblationStudies}


We performed ablation studies to isolate the contribution of various techniques used to increase classification performance.

These techniques are 
\begin{itemize}
\item dimensionality reduction features
\item histogram comparison features
\item synthetic augmentation of feature vectors
\item range normalization of feature vectors
\item weakened strain boosting of poor-performing attack classes
\item clustering often confounded attack classes
\end{itemize}


To evaluate the performance of the detector and the classifier, we first will focus on F1 score for natural samples ($C0$-$F1$) and the macro-averaged F1 score across the various attacks ($AVG$-$F1$). We also compare the average and maximum accuracies ($MuAcc, MxAcc$) reported for classification as well as detection ($CLF$, $DTC$) modes.

The ablation studies below itemize the contribution of these techniques to increase in accuracy metrics of interest. 









\subsection{Impact of Doubling The Data}
 Will our detector respond well to an increase of training data? Next, we doubled the initial 5000 CIFAR-10 samples data, resulting in a total of  $(N=10000)\dot (13+1)$ samples. Our initial baseline used 5000 CIFAR-10 samples and subjected them to the 13 attack classes, generating $(N=5000)\dot (13+1)$ samples for our second stage classifier. The following ablation shows the impact of doubling the available data over accuracy metrics. The remainder of experiments rely on N=10000.





\subsection{Earth Moving Distances}

Wasserstein distances or so-called earth moving distances techniques to estimate work needed to make make-alike two distributions.

In a nutshell, Wasserstein distance is a measure of the optimal effort to make two binned distributions become alike. Lower values represent similarly binned distributions, higher distributions for which significant shaping work is needed to make them alike. We use 23 bins.

The following ablation table compares detection and classification accuracy metrics between basic fine-grained features versus fine-grained features plus distributional shape features obtained using Wasserstein distances (also referred to as earth moving distances). The extra features yield a very modest $1\%$ increase on accuracy metrics.


\input{TABLES/table_extrafeatures}






\subsection{Dimensionality Reduction Features}
We use a fine-grained anomaly detection feature space --- some features being correlated and/or redundant. It is worth to examine if dimensionality reduction techniques will enhance our performance. 







Principal Component Analysis (PCA) and Linear Discriminant Analysis (LDA) techniques can be used to introduce proxy features that capture most of the variability or reduce most of the cross entropy. While it is known that these proxy features are a gamble and can in general these features can hurt accuracy metrics, could it possible that they will contribute positively in differentiating between two distributions?

The following ablation table compares detection and classification accuracy metrics between normal, PCA-augmented, LDA-augmented and PCA and LDA augmented runs. Under the non-clustered mode, PCA adds again a modest $1\%$ increase in performance, whether LDA is used or not.

\input{TABLES/table_pcalda}





\subsection{Synthetic Data Augmentation}
Generative techniques to randomly sample a minute epsilon-ball around the point ascribed to an input feature vector. By choosing a very minute epsilon, we speculate the label of these samples to be the same as the input sample and generate additional samples to drive up robustness of the neural network with respect to minute perturbations on the underlying input feature vector.

We investigated whether by synthetically augmenting our dataset, we could increase accuracy metrics. Specifically, we introduced a very small noise perturbation around each feature value of a sample's profile. An adversarial attack essentially perturbs samples but with the optimization goal of switching the classifier's label. On the other hand, we introduce minute noise, but to expand the recognition range of the resulting classifier towards slightly perturbed samples. The perturbations of the (statistical profile) feature vector for the $i^{th}$ sample (with elements $x_{ij}$ was of the form 
\begin{equation}
    x^*_{ij} = x_{ij} \pm (\sigma_{j} \* \rho_{j} \* \epsilon + \eta_{ij})
\end{equation}
where $\sigma_j$ corresponds to the standard deviation for the population of the given feature $x_j$, $\rho$ is a random magnitude in the range $[-1, 1]$ and $\epsilon$ the scaling factor of the resulting perturbation (e.g., $10^{-10}$).

The following ablation table compares detection and classification accuracy metrics between the synthetic augmentation at various $\epsilon$ values in the range $[10^{-6}, 10^{-15}]$.

\input{TABLES/table_aug}

\input{TABLES/table_augeps}






% \subsection{Impact of Normalization Techniques}
% A number of techniques can be use to normalize the input variables with standard scaler often use in anomaly detection because it separates outliers from normal samples, however, numerical stability is better achieved through unit normalization although a loss in outlier signal is induced.

% The following ablation table compares detection and classification accuracy metrics between anomaly-oriented scaling and stability-oriented scaling.

% \input{TABLES/table_minmaxscaler}




\subsection{Robustness via Weakened Strains}
In constructing the attack samples, each attack is applied over the set of natural samples using basic or default parameters. Each natural sample has two possible outcomes: successfully attacked or failed attack. The following table itemizes for each class, how many natural samples were processed, how many were successfully attacked, how many were failed attacks and what was the resulting accuracy metrics for the attack class during evaluation mode.

Each attack could be made harsher or be weakened. Using a metaphor of immunization, where a weakened strain is used to help the immune system ML to learn to detect and target such viruses, for attack classes were we obtained low detection/classification performance, we double the data with similarly generated attack samples but using weakened parameters. The following table shows the increase in accuracy metrics obtained in classification/detection for each of these attacks and the overall increase in classification and detection accuracy metrics.








\subsection{Handling of Failed Attacks}
What to do with failed attack samples?
A failed attack sample could lie anywhere within close proximity to the successful new class label or just the opposite, towards close proximity to the natural sample's label. In the case of the former, it is detrimental to the classification margin/boundary to include this sample as representative of the attack class -- as it pushes the attack membership towards the natural/clean cluster. This problem requires either dropping the failed attacks, including them into the attack class, or a mix of these two based on some clustering criteria.








\subsection{Best Classification Performance}
\input{TABLES/table_best}






\subsection{Experiment Control Parameters}
Declaw allows command line user-control of the application of these various hypothesis that expand the basic anomaly feature vector. These parameters are shown in Table~\ref{tab:controlparameters}.


\input{TABLES/table_controlparameters}




Declaw also provides user control of various basic hyper-parameters. These parameters are shown in Table~\ref{tab:hyperarameters}.



\input{TABLES/table_hyperparameters}



==> 12_attacking.tex <==

\section{Attacking the Defense}
\label{Section:AttackingTheDetector}

Finally, we analyze the performance of a white box iterative attack.

Using Carlini amd Warner's approach, we attacked the detector by incorporating into the gradient recomputation of the first state attack, a cross-entropy term against the second stage detector's logit prediction.




==> 13a_future_work.tex <==

\section{Future Work}
\label{Section:FutureWork}

\subsection{Adaptive attacks}
One limitation of this work is the lack of adaptive attack evaluation. Prior work shows that previous detectors can be attacked with adaptive attacks~\cite{carlini2017adversarial}. While we use a lot of statistical profiling in our AFVs, it remains to be seen how an adaptive adversary would perform.

\subsection{Handling of Out of Distribution Inputs}
The validation and/or certification of inputs is of importance to both training as well as evaluation tasks.




\begin{itemize}
    \item During training- it will be desirable to know if samples represent out-of-distribution instances or even if the classification support for these is too small. The former is typically associated with population-based anomaly detection limits while the latter is associated with whether the sample's anomaly-detection feature vector aligned to a known cluster, centroid or representative sample in the feature space.

    \item During evaluation- it will be desirable to reliably distinguish between samples suspected to be compromised by an attack and decide whether to reject the sample, log and trace the anomaly, ignore the attack or perhaps reroute the sample to a more robust classifier.
\end{itemize}




\subsection{Concept Shift}
Our approach relies on a single reference temperature (i.e., representative sample or centroid) for the entire natural samples dataset. However, this could be made more robust. Specifically, two simple but very important enhancements could be made. 
\begin{itemize}
    \item removal of outliers: the dataset of natural samples may contain extreme outliers that could bias or even nullify the computation of the reference temperature for the overall dataset (i.e., a series of fine-grained centroid computations). We could first perform a first pass over the dataset of natural samples and compute an initial reference temperature, then identify any anomalous natural samples with respect to this initial reference temperature (e.g., plus/minus three sigma from the our first reference temperature estimators) and then recompute the final reference temperature on a second pass over the set of non-anomalous natural samples.
    
    \item multimodal distributions: the dataset of natural samples could manifest a multimodal distribution with respect to our features. Visually, this  represents the case where the anomaly detection feature vectors for natural samples do not cluster into one well-defined Gaussian multivariate cluster but rather into two or more clusters. A representative sample for both could be misleading or meaningless (e.g., cluster one represents daylight conditions and cluster two represents nighttime conditions). Trivially, one could use multiple detectors for expressing these ultimately different concepts. Alternatively, our second stage network architecture could be extended to explicitly learn such user-provided or domain-related features of importance to the classification.
    
\end{itemize}

    
\subsection{Large Number of Classes}
There is no reason for generating and partitioning anomaly feature vectors classification classes solely on attack method. Thanks to our clustering methodology, it is possible to train a large cardinality classifier where dozens classes to express variants of a given attack method are used (e.g., $PGD3, PGD10, PGD20, PGD40$, etc). Similarly, it might be desirable to express a class for failed versions of attacks, which are expected to have a different distribution to that of successful attacks. Same principles apply to addressing multimodal natural samples.
    



\subsection{Healing of damaged or attacked samples}
By leveraging the concepts of a representative sample and a normative subset of natural samples, we can explore the concept of automatically healing anomalous values in the observed layer values $l^*_i$ that exceed a strong anomaly $hi$ watermark (e.g.
$\mu + 3\sigma$). The autonomous healing comprises a weighted function of the actual pixel value plus the corresponding element wise value from the normative baseline. 

==> 15_bibliography.tex <==


\bibliographystyle{unsrt}

\begin{thebibliography}{00}
% \bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
% \bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
% \bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
% \bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
% \bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
% \bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
% \bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989





\bibitem{metzen2017detecting}
      Jan Hendrik Metzen and Tim Genewein and Volker Fischer and Bastian Bischoff,
      ``On Detecting Adversarial Perturbations,''
      arXiv, 1702.04267, stat.ML, 2017.



\bibitem{croce2020reliable}
      Francesco Croce and Matthias Hein,
        ``Reliable evaluation of adversarial robustness with an ensemble of diverse parameter-free attacks,''
        arXiv, 2003.01690, cs.LG, 2020.




\bibitem{andriushchenko2020square}
    Maksym Andriushchenko and Francesco Croce and Nicolas Flammarion and Matthias Hein,
    ``Square Attack: a query-efficient black-box adversarial attack via random search,''
      arXiv, 1912.00049, cs.LG, 2020.




\bibitem{engstrom2019exploring}
    Logan Engstrom and Brandon Tran and Dimitris Tsipras and Ludwig Schmidt and Aleksander Madry,
      ``Exploring the Landscape of Spatial Robustness, ''
       arXiv, 1712.02779, cs.LG, 2019.




\bibitem{carlini2017evaluating}
      title={}, 
      Nicholas Carlini and David Wagner,
      ``Towards Evaluating the Robustness of Neural Networks,''
    
    

\bibitem{moosavidezfooli2016deepfool}
      Seyed-Mohsen Moosavi-Dezfooli and Alhussein Fawzi and Pascal Frossard,
    ``DeepFool: a simple and accurate method to fool deep neural networks,'' 
      arXiv, 1511.04599, cs.LG, 2016.



@misc{pang2018robust,
      title={Towards Robust Detection of Adversarial Examples},
      author={Tianyu Pang and Chao Du and Yinpeng Dong and Jun Zhu},
      year={2018},
      eprint={1706.00633},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}


@misc{cohen2020detecting,
      title={Detecting Adversarial Samples Using Influence Functions and Nearest Neighbors},
      author={Gilad Cohen and Guillermo Sapiro and Raja Giryes},
      year={2020},
      eprint={1909.06872},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}


@misc{papernot2018deep,
      title={Deep k-Nearest Neighbors: Towards Confident, Interpretable and Robust Deep Learning},
      author={Nicolas Papernot and Patrick McDaniel},
      year={2018},
      eprint={1803.04765},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

\end{thebibliography}



==> FIGURES/figure.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

==> FIGURES/table <==
\hline
name & precision  & recall  & f1-score  &  support
\hline
00  &                    clean  & .60 & .65 & .62 \\
\hline
01 &                  apgd_ce  & .96 & .89 & .92 \\
02 &                 apgd_dlr  & .73 & .67 & .70 \\
03 &                bb_square  & .29 & .35 & .32 \\
04 &ev_basic_iterative_method  & .94 & .93 & .94 \\
05 &     ev_carliniwarner_inf  & .24 & .14 & .18 \\
06 &      ev_carliniwarner_l2  & .24 & .22 & .23 \\
07 &              ev_deepfool  & .33 & .20 & .25 \\
08 &                   ev_fgm  & .99 & .99 & .99 \\
09 &           ev_hopskipjump  & .29 & .39 & .34 \\
10 &            ev_newtonfool  & .48 & .48 & .48 \\
11 &    ev_spatial_transforms  & .00 & .00 & .00 \\
12 &           ev_wasserstein  & .51 & .82 & .63 \\
13 &                      pgd  & .88 & .92 & .90 \\
\hline
\hline
                 accuracy  &     &     & .61 \\
                macro avg  & .60 & .62 & .61 \\
             weighted avg  & .61 & .61 & .61 \\
\hline



==> TABLES/table_aug.tex <==


% NON CLUSTERED
\begin{table}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
LR & AUG & C0 & AVG & DET & CLF & N  \\
  & & F1 & F1 & MuACC & MuACC &  \\
\hline
\hline
 0.01 & 0   & 0.905 & 0.92   & 0.926     & 0.734     & 51  \\
 0.01 & 1   & 0.912 & 0.93   & 0.933     & 0.751     & 86  \\
 \hline
 1.0  & 0   & 0.93  & 0.945  & 0.948     & 0.788     & 255 \\
 1.0  & 1   & 0.932 & 0.949  & 0.949     & 0.792     & 243 \\
\hline
\end{tabular}
\caption{\bf{Is there Any Benefit to Data Augmentation?} We examine whether synthetic data augmentation increased F1 scores for natural samples $F1_{C}$, the micro-averaged F1 $F1_{C+A_k}$ across classes, or even average DETECTION accuracy and CLASSIFICATION accuracy -- when averaged across many runs of a grid hyper-parameter space. The number of evaluations used to average the estimate is $N$. The synthetic data augmentation contributes a $1\%$ increase in the F1 score for natural samples and a $1\%$ across classes when sub-optimal learning rates are used.}
\end{table}














==> TABLES/table_augeps.tex <==
\begin{table}
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
EPS  & C0 & AVG & DET & CLF & N  \\
   & F1 & F1 & MuACC & MuACC &   \\
   \hline
   \hline
 1e-06 & 0.907 & 0.927  & 0.929     & 0.75      & 3  \\
 1e-07 & 0.91  & 0.93   & 0.931     & 0.751     & 3  \\
 1e-08 & 0.917 & 0.93   & 0.935     & 0.751     & 3  \\
 1e-09 & 0.917 & 0.93   & 0.935     & 0.75      & 6  \\
 1e-10 & 0.917 & 0.93   & 0.935     & 0.752     & 3  \\
 1e-11 & 0.911 & 0.93   & 0.933     & 0.751     & 56 \\
 1e-12 & 0.913 & 0.93   & 0.935     & 0.75      & 3  \\
 1e-13 & 0.917 & 0.93   & 0.935     & 0.75      & 3  \\
 1e-14 & 0.91  & 0.93   & 0.934     & 0.752     & 3  \\
 1e-15 & 0.913 & 0.93   & 0.935     & 0.75      & 3  \\
\hline
\end{tabular}
\caption{\bf{How stable is the synthetic data augmentation across various perturbation epsilon values?} The technique delivers stable results the plateau $[1e^{-7}, 1e^{-15}$ --- i.e, a wide range of epsilon values.}
\end{table}

==> TABLES/table_best.tex <==


% NON CLUSTERED
\begin{table}[t]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
  LR   & AUG & C0 & AVG & DET & CLF &  N  \\
     &  & F1 & F1 & MuACC & MuACC &    \\
\hline
\hline
 0.01 & 0   & 0.905 & 0.92   & 0.926     & 0.734     & 51  \\
 0.01 & 1   & 0.912 & 0.93   & 0.933     & 0.751     & 86  \\
 1.0  & 0   & 0.93  & 0.945  & 0.948     & 0.788     & 255 \\
 1.0  & 1   & 0.932 & 0.949  & 0.949     & 0.792     & 243 \\
\hline
\end{tabular}
\caption{\bf{Non Clustered Mode Best Performance:} Best performing parameter combinations by F1 values for natural samples and micro-averaged F1 values across all classes. Using this criteria, all models are in a plateau, whose maximal point is $96.3\%$ for detection $Acc_{C|A_k}$ and $80.0\%$ for classification $Acc_{C|A_*}$ for our baseline setup of detecting 11 different attacks.}
\end{table}





==> TABLES/table_cifar10.tex <==
\begin{table}
\begin{tabular}{|l|p{2.7in}|}
\hline
Layer & SamplingHookModel( \\
\hline
($model$) & WideResNet( \\
($conv_1$) & Conv2d(3, 16, kernel=(3,3), stride=(1,1), pad=(1,1), bias=F)\\
\hline
($block_1$) & NetworkBlock( \\
($layer$) &  Sequential(BasicBlock(160) x 5)) \\
\hline
($sublk_1$) & NetworkBlock( \\
($layer$) & Sequential(BasicBlock(160) x 5)) \\
\hline
($block_2$) & NetworkBlock( \\
($layer$) & Sequential(BasicBlock(160) x 1, BasicBlock(320) x 4)) \\
\hline
($block_3$) & NetworkBlock( \\
($layer$) &  Sequential(BasicBlock(320) x 1, BasicBlock(640) x 4)) \\
\hline
***
($bn_1$) & BatchNorm2d(640, eps=1e-05, mom=0.1, aff=T, track=T)\\
\hline
($RELU$) & ReLU(inplace=True) \\
\hline
($FC$) & Linear(in=640, out=10, bias=T)) \\
\hline
\end{tabular}
\caption{Placeholder for WideResNet Model Figure Showing Sampling Hook inherited by Subclassing and showing the place of the Batch Normalization Layer being sampled being at the end of the pipeline.}
\end{table}

==> TABLES/table_controlparameters.tex <==


\begin{table}[t]
    \centering
    \begin{tabular}{|l|l|l|p{1.1in}|}
    \hline
Parameter & Values & Default & Description \\
\hline
\hline
data\_augment                  & True/False            & 1                     & apply robust data augmentation \\
\hline
cluster\_mode                  & True/False            & 0                     & cluster similar attacks? \\
\hline
eval\_mode                     & True/False            & 0                     &  evaluation mode \\
\hline
use\_knn                       & True/False            & 1                     & estimate classification support \\
\hline
use\_lda                       & True/False            & 1                     & add LDA features \\
\hline
use\_pca                       & True/False            & 0                     & add PCA features \\
\hline
extra\_features                & $0, 1, 2, 3, 4$       & 1                     & add EMD features \\
\hline
augment\_eps                   & $[1e^{-6}, 1e^{-15}]$       & $1e^{-11} $               & data augmentation $\epsilon$\\
\hline

                                  
    \end{tabular}
    \caption{Declaw's experiment control parameters.}
    \label{tab:controlparameters}
\end{table}





==> TABLES/table_declaw_model.tex <==
\begin{table}
\begin{tabular}{|l|p{2.6in}|}
\hline
Layer & Model Multiclass Classification( \\
\hline
($layer_1$) & Linear(in=190, out=800, bias=True) \\
($BN_1$) & BatchNorm1d(800, eps=1e-05, mom=0.1, aff=F, stats=T) \\
\hline
($layer_2$) & Linear(in=800, out=400, bias=True) \\
($BN_2$) & BatchNorm1d(400, eps=1e-05, mom=0.1, aff=F, stats=T) \\
\hline
($layer_3$) & Linear(in=400, out=200, bias=True) \\
($BN_3$) & BatchNorm1d(200, eps=1e-05, mom=0.1, aff=F, stats=T) \\
\hline
($layer_4$) & Linear(in=200, out=100, bias=True) \\
($BN_4$) & BatchNorm1d(100, eps=1e-05, mom=0.1, aff=F, stats=T) \\
\hline
($layer5$) & Linear(in=100, out=50, bias=True) \\
($BN_5$) & BatchNorm1d(50, eps=1e-05, mom=0.1, aff=F, stats=T) \\
\hline
($layer_{out}$) & Linear(in=50, out=14, bias=True)\\
($RELU$) & LeakyReLU(negslope=0.01) \\
\hline
($dropout_{hi}$) & Dropout(p=0.1667, inplace=False) \\
($dropout_{lo}$) & Dropout(p=0.0417, inplace=False) \\
\hline
\hline
\end{tabular}
\label{declaw_stages}
\caption{Placeholder for Classification/ Detection  Model}
\end{table}

==> TABLES/table_extrafeatures.tex <==
\begin{table}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
  LR   & EXTR & C0 & AVG & DET & CLF &  N  \\
     & FEAT & F1 & F1 & MuACC & MuACC &    \\
\hline
\hline
 0.01 & 0    & 0.907 & 0.926  & 0.93      & 0.743     & 44 \\
 0.01 & 1    & 0.91  & 0.926  & 0.931     & 0.746     & 49 \\
 0.01 & 2    & 0.911 & 0.926  & 0.931     & 0.745     & 44 \\
\hline
\end{tabular}
\caption{\bf{Do fine-grained distribution features impact the accuracy metrics targeted?} Our current earth moving distances do not contribute atop the existing histogram features. They contribute minimally when suboptimal learning rates are used.}
\end{table}

==> TABLES/table_feature_importances.tex <==
\begin{table*}
\centering
\begin{tabular}{|l|l|l||}
\hline

FEATURE & IMPORTANCES & DESCRIPTION \\

\hline
p\_normally\_distr &    0.04932 & p-value from testing whether $x^*_i$ values are normally distributed\\

p\_same\_means\_hat &    0.04449 & p-value estimate from testing whether $x^*_i$ values have same mean as $x^C_i$ values\\

p\_same\_means\_pnt &    0.05013 & p-value from testing whether $x^*_i$ values have same mean as $x^C_i$ values\\

p\_same\_dist &    0.03951 & p-value from testing whether $x^*_i$ values have same distribution as $x^C_i$ values\\

p\_same\_variance &    0.02882 & p-value from testing whether $x^*_i$ values have same variance as $x^C_i$ values\\

\hline
key\_metric &    0.00320 & description \\

(n\_errors/n) &    0.00352 & average number of anomalies across the population of $x^*_i$ compared against $x^C_i$ values\\

right &    0.00310 & number of anomalies on the $S_{RI}$ region\\

left &    0.00337 & number of anomalies on the $S_{LE}$ region \\

overall &    0.00407 & number of anomalies in the $S_{OV}$ region \\

\hline
(right/overall) &    0.00242 & ratio of $cnt(S_{RI})/cnt{S_OV}$ \\

(left/overall) &    0.00889 & \\

((right-left)/overall) &    0.00155 & description \\

\hline
((z*right).sum()) &    0.00331 & sum of z-scores for $x^*_i$ values on the $S_{RI}$ region\\

((z*left).sum()) &    0.00302 & description \\

(z.sum()) &    0.00387 & description \\

\hline
((z*right).sum()/n) &    0.00416  & average of z-scores for $x^*_i$ values on the $S_{RI}$ region \\

((z*left).sum()/n) &    0.00352 &  description \\

(z.sum()/n) &    0.00447 & description \\

\hline
(anomaly\_err) &    0.00004 & description \\

(within\_err) &    0.00274& description  \\

(total\_err) &    0.00277& description  \\

\hline
(anomaly\_err/within\_err) &    0.00856 & description  \\

(anomaly\_err/n\_errors) &    0.00264& description  \\

(within\_err/(n-n\_errors+1)) &    0.00336& description  \\

\hline
(within\_err/total\_err) &    0.00139 & description \\
(total\_err/n) &    0.00213 & description \\

\hline
avg\_anomaly\_zscore &    0.00228 & description \\

avg\_within\_zscore &    0.00912 & description \\

avg\_zscore &    0.00869 & description  \\

\hline
score &    0.00935 & description \\

norm\_score &    0.01123 & description \\

\hline
f0 - f22 &    min=0.0002, avg=0.01096, max=0.0204 & 23 flags with respect to various extrema detection\\

\hline
s0 - s22 & min=0.0001, avg=0.0004, max=0.0014 & histogram bin counts for the distribution of $x^*_i$ values \\

\hline
q0 - q22 & min=0.0005, avg=0.0023, max=0.0096 
& square of the difference between $x^*_i$ values and the expected $x^C_i$ natural values \\

\hline
r0 - r22 & min=0.0005, avg=0.0034, max=0.0122 & relative error between observed $x^*_i$ values and expected $x^C_i$ values \\

\hline
rsum &    0.00077 & sum of all the relative errors above \\

rvar &    0.00112  & variance of all relative errors above\\

rmean &    0.00159 & average of all relative errors above \\

\hline
\hline
\end{tabular}
\caption{Feature generated by the SamplingHook. The DeClaW classifier generates some additional features derived from these, most prominently, distribution (e.g., shape, tail, area, symmetry) comparison features. Feature importance shown for initial features using CLF Random Forest($max_{depth}=16$, $max_{feat}=16$, n=200)}
\end{table*}







==> TABLES/table_knn.tex <==
\begin{table}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
 LR  &  KNN  & C0 & AVG & DET & CLF &  N  \\
    &    & F1 & F1 & MuACC & MuACC &    \\
\hline
\hline
 0.01 & 0     & 0.914 & 0.929  & 0.933     & 0.749     & 37 \\
 0.01 & 2500  & 0.91  & 0.93   & 0.934     & 0.752     & 1  \\
 0.01 & 5000  & 0.908 & 0.925  & 0.929     & 0.743     & 96 \\
 0.01 & 10000 & 0.91  & 0.93   & 0.931     & 0.753     & 1  \\
 0.01 & 20000 & 0.91  & 0.93   & 0.93      & 0.754     & 1  \\
 0.01 & 50000 & 0.9   & 0.92   & 0.921     & 0.753     & 1  \\
\hline
\end{tabular}
\caption{}
\end{table}

==> TABLES/table_minmaxscaler.tex <==
\begin{table}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
  LR   & SCA & C0 & AVG & DET & CLF &  N  \\
     &  & F1 & F1 & MuACC & MuACC &    \\
\hline
\hline
 0.001 & 1   & 0.908 & 0.926  & 0.93      & 0.646     & 16  \\
 0.001 & 0   & 0.911 & 0.928  & 0.931     & 0.67      & 20  \\
 \hline
 0.01  & 1   & 0.937 & 0.949  & 0.952     & 0.746     & 16  \\
 0.01  & 0   & 0.941 & 0.951  & 0.955     & 0.758     & 20  \\
\hline
 1.0   & 1   & 0.95  & 0.96   & 0.962     & 0.797     & 84  \\
 1.0   & 0   & 0.95  & 0.96   & 0.963     & 0.8       & 100 \\
 \hline
\end{tabular}
\caption{\bf{Should a scaler for anomaly detection or a scaler for numerical stability be used?} An anomaly oriented scaler (i.e., the standard scaler) brings an average benefit of $1\%$ to the observed average classification accuracy.}
\end{table}

==> TABLES/table_pcalda.tex <==
\begin{table}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
  LR  & P & L & A & C0 & AVG & DET & CLF &  N \\  
    &  C&  D&  U& F1 & F1 & MuACC & MuACC &  \\
    &  A&  A&  G&  &  &  &  &  \\
\hline
\hline
 0.01 & 1   & 0   & 0   & 0.903 & 0.92   & 0.925     & 0.734     & 12 \\
 0.01 & 0   & 0   & 0   & 0.905 & 0.92   & 0.926     & 0.733     & 15 \\
 0.01 & 0   & 1   & 0   & 0.906 & 0.92   & 0.926     & 0.735     & 12 \\
 0.01 & 1   & 1   & 0   & 0.907 & 0.92   & 0.926     & 0.734     & 12 \\
 \hline
 0.01 & 1   & 0   & 1   & 0.91  & 0.93   & 0.933     & 0.751     & 12 \\
 0.01 & 0   & 0   & 1   & 0.914 & 0.93   & 0.934     & 0.751     & 45 \\
 0.01 & 0   & 1   & 1   & 0.911 & 0.93   & 0.933     & 0.751     & 12 \\
 0.01 & 1   & 1   & 1   & 0.911 & 0.929  & 0.932     & 0.752     & 17 \\
\hline
\end{tabular}
\caption{\bf{Is there any benefit to the use of Dimensionality Reduction Features to our anomaly detection?}. Dimensionality reduction features do not significantly contribute, on the average, to an increase on the metrics we tracked.}
\end{table}

==> TABLES/table_profile_natural.tex <==
\begin{table*}
\centering
\begin{tabular}{|l|r|r|r|r|r|}
\hline
anomaly feature($f_k$)                          & $LCL(f_k)$    & $\mu_{f_k}$ &  $\mu_{x_i|f_k}$ & $UCL(f_k)$ & Outcome      \\
\hline
n_errors                                        &  40227.771 <= & 40300.796&    40377.0& <=  40373.822 &      False\\ 
((n-n_errors)/n)                                &      0.014 <= &     0.016&      0.014& <=      0.018 &      False\\ 
(n_errors/n)                                    &      0.982 <= &     0.984&      0.986& <=      0.986 &      False\\ 
\hline
right                                           &  16710.664 <= & 18865.788&    21801.0& <=  21020.912 &      False\\ 
left                                            &  19254.174 <= & 21435.009&    18576.0& <=  23615.843 &      False\\ 
overall                                         &  40228.771 <= & 40301.796&    40378.0& <=  40374.822 &      False\\ 
\hline
(right/overall)                                 &      0.414 <= &     0.468&       0.54& <=      0.522 &      False\\ 
(left/overall)                                  &      0.478 <= &     0.532&       0.46& <=      0.586 &      False\\ 
((right-left)/overall)                          &     -0.171 <= &    -0.064&       0.08& <=      0.044 &      False\\ 
\hline
((z*right).sum())                               & 940696 <= &1068603& 1268760.534& <= 1196510 &      False\\ 
((z*left).sum())                                &  814890 <= &1069760& 953551.236& <= 1324630 &       True\\  
(z.sum())                                       & 1908421 <= &2138693& 2222610.25& <= 2368966 &       True\\  
\hline
((z*right).sum()/n)                             &   1469.839 <= &  1669.693&   1982.438& <=   1869.547 &      False\\ 
((z*left).sum()/n)                              &   1273.267 <= &  1671.501&   1489.924& <=   2069.735 &       True\\  
(z.sum()/n)                                     &   2981.908 <= &  3341.709&   3472.829& <=    3701.51 &       True\\  
\hline
(anomaly_err)                                   & 1908065.572 <= &2138364.004&  2222311.5& <= 2368662.435 &       True\\  
(within_err)                                    &    292.303 <= &   329.625&    298.418& <=    366.947 &       True\\  
(total_err)                                     & -332218.893 <= & -1159.506&  315202.44& <= 329899.881 &       True\\  
\hline
(anomaly_err/within_err)                        &   5279.636 <= &  6627.091&    7447.97& <=   7974.546 &       True\\  
(anomaly_err/n_errors)                          &     47.404 <= &    53.052&     55.038& <=     58.699 &       True\\  
(within_err/(n-n_errors+1))                     &      0.488 <= &     0.499&      0.511& <=      0.511 &      False\\ 
(within_err/total_err)                          &     -0.003 <= &     0.073&      0.001& <=      0.004 &       True\\  
\hline
(total_err/n)                                   &     -8.111 <= &    -0.028&      7.695& <=      8.054 &       True\\  
\end{tabular}
\caption{Anomaly profile for NATURAL sample evaluated at $1\sigma$ control limits -- derived from NATURAL samples dataset.}
\end{table*}

==> TABLES/table_profile_pgd20.tex <==
\begin{table*}
\centering
\begin{tabular}{|l|r|r|r|r|r|}
anomaly feature($f_k$)                          & $LCL(f_k)$    & $\mu_{f_k}$ &  $\mu_{x_i|f_k}$ & $UCL(f_k)$ & Outcome      \\
nerrs                                        &  40227.771 <= & 40300.796 &    40452.0 & <=  40373.822 &      False \\
((n-nerrs)/n)                                &      0.014 <= &     0.016 &      0.012 & <=      0.018 &      False \\
(nerrs/n)                                    &      0.982 <= &     0.984 &      0.988 & <=      0.986 &      False \\
\hline
right                                           &  16710.664 <= & 18865.788 &    22322.0 & <=  21020.912 &      False \\
left                                            &  19254.174 <= & 21435.009 &    18130.0 & <=  23615.843 &      False \\
overall                                         &  40228.771 <= & 40301.796 &    40453.0 & <=  40374.822 &      False \\
\hline
(right/overall)                                 &      0.414 <= &     0.468 &      0.552 & <=      0.522 &      False \\
(left/overall)                                  &      0.478 <= &     0.532 &      0.448 & <=      0.586 &      False \\
((right-left)/overall)                          &     -0.171 <= &    -0.064 &      0.104 & <=      0.044 &      False \\
\hline
((z*right).sum())                               & 940696.951 <= &1068603 & 1768072.412 & <= 1196510 &      False \\
((z*left).sum())                                &  814890.81 <= &1069760  & 943103.279 & <= 1324630 &       True \\
(z.sum())                                       & 1908421.152 <=&(2138693 &  2711428.5 & <= 2368966 &      False \\
\hline
((z*right).sum()/n)                             &   1469.839 <= &  1669.693 &   2762.613 & <=   1869.547 &      False \\
((z*left).sum()/n)                              &   1273.267 <= &  1671.501 &   1473.599 & <=   2069.735 &       True \\
(z.sum()/n)                                     &   2981.908 <= &  3341.709 &   4236.607 & <=    3701.51 &      False \\
\hline
(anomaly_err)                                   & 1908065 <=&2138364 &  2711175.5 & <= 2368662 &      False \\
(within_err)                                    &    292.303 <= &   329.625 &    252.831 & <=    366.947 &      False \\
(total_err)                                     & -332218.893 <=& -1159.506 &  824968.94 & <= 329899.881 &      False \\
\hline
(anomaly_err/within_err)                        &   5279.636 <= &  6627.091 &  10724.293 & <=   7974.546 &      False \\
(anomaly_err/n_errors)                          &     47.404 <= &    53.052 &      67.02 & <=     58.699 &      False \\
(within_err/(n-n_errors+1))                     &      0.488 <= &     0.499 &      0.497 & <=      0.511 &       True \\
(within_err/total_err)                          &     -0.003 <= &     0.073 &        0.0 & <=      0.004 &       True \\
\hline
(total_err/n)                                   &     -8.111 <= &    -0.028 &     20.141 & <=      8.054 &      False \\
\end{tabular}
\caption{Anomaly profile for PGD20 sample evaluated at $1\sigma$ control limits -- derived from NATURAL samples dataset.}
\end{table*}



==> afv_components.tex <==
AFVs are composed of these anomaly detection features (see Appendix~\ref{Section:Formulation}.
%\rf{each of the features used to create the anomaly feature vector should be defined clearly in the approach section of the paper (e.g., how exactly do I form the 25 region-based features and so on) but in the introduction a broad categorization of the types of features used should suffice}:
       \begin{itemize}
        \item $25$ region-based features (e.g., left tail, right tail, center area, entire area) to characterize various subsampling projections of the distribution of observed layer input values:\\ $f_{1}(l^{*}_i) \cdots f_{25}(l^{*}_i)$.
        \item $25$ extrema-based features to characterize whether observed metrics above represent statistical outliers with respect to the upper (e.g., $90\%$) and lower (e.g., $10\%$) percentiles of the expected distribution of natural samples: $f_{26}(l^{*}_i) \cdots f_{50}(l^{*}_i)$.
        \item $23$ observed bincount features: $f_{51}(l^{*}_i) \cdots f_{73}(l^{*}_i)$.
        \item $69$ comparative features that compare observed bincounts vs expected bincounts for normative natural samples: \\$f_{74}(l^{*}_i) \cdots f_{142}(l^{*}_i)$.
        \item $5$ A/B probability tests features: $f_{143}(l^{*}_i) \cdots f_{147}(l^{*}_i)$.
        \item $10$ Wasserstein distance features used to compare the shape and area of tails of the observed distribution against the distribution of normative natural samples : $f_{148}(l^{*}_i) \cdots f_{157}(l^{*}_i)$.
        \item $6$ PCA/LDA dimensionality projection features:\\ $f_{158}(l^{*}_i) \cdots f_{163}(l^{*}_i)$.
        \item $12$ KNN features used to estimate classification support for a given sample based on a $3\sigma$ based neighborhood:\\ $f_{164}(l^{*}_i) \cdots f_{175}(l^{*}_i)$.
        \end{itemize}



These features provide robust representations of layer input values, over which comparative analyses are performed between observed values vs expected values for normative natural samples.%\footnote{Though these features are sufficient to surpass accuracy metrics of previous research, we foresee that kernel/convolution features would be needed for a few attacks that closely mimic the distribution of natural samples.}
